Kernel Machines Beat Deep Neural Networks on Mask-based Single-channel Speech Enhancement

We apply a fast kernel method for mask-based single-channel speech enhancement. Specifically, our method solves a kernel regression problem associated to a non-smooth kernel function (exponential power kernel) with a highly efficient iterative method (EigenPro). Due to the simplicity of this method, its hyper-parameters such as kernel bandwidth can be automatically and efficiently selected using line search with subsamples of training data. We observe an empirical correlation between the regression loss (mean square error) and regular metrics for speech enhancement. This observation justifies our training target and motivates us to achieve lower regression loss by training separate kernel model per frequency subband. We compare our method with the state-of-the-art deep neural networks on mask-based HINT and TIMIT. Experimental results show that our kernel method consistently outperforms deep neural networks while requiring less training time.

==> figs/multiband.tex <==
% \begin{figure}[htb]
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{multiK.jpg}
%   \caption{Factory1 -5dB}
%   \label{fig:fac -5}
% \end{subfigure}%
% \end{figure}
% \begin{figure}[htb]
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{kernel_func1.jpg}
%   \caption{different kernels}
%   \label{fig:kernel func}
% \end{subfigure}
% \caption{(a-c): MSE along per frequency subband}
% \label{fig:test}
% \end{figure}
\begin{wrapfigure}{r}{.25\textwidth}
  \vspace{-5mm}
  \includegraphics[width=\linewidth]{figs/multiK.jpg}
    \vspace{-5mm}
\caption{Factory1 -5dB}
  \label{fig:fac -5}
\vspace{-3mm}
\end{wrapfigure}

==> figs/multiband_and_kernels.tex <==
\begin{figure}[!ht]
\begin{minipage}{.25\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/multiK.jpg}
    \vspace{-5mm}
\caption{Factory1 -5dB}
  \label{fig:fac -5}
\end{minipage}
\begin{minipage}{.25\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/kernel_func.jpg}
    \vspace{-5mm}
\caption{Smoothness of kernels}
  \label{fig:kernels}
\end{minipage}
\end{figure}

==> figs/ssn0.tex <==
\begin{wrapfigure}{r}{.25\textwidth}
  \vspace{-3mm}
  \includegraphics[width=.25\textwidth]
%   {figs/kernel_func.jpg}
  {figs/ssn0.png}
\vspace{-7mm}
\end{wrapfigure}

==> soft-thresh.tex <==
% We use a dispersal (power) kernel \cite{nathan2006long}, which has an adaptive power value $\gamma$, as in 
% \begin{center}
% $k_{\gamma, \sigma}(\bm{x}, \bm{z}) = exp(-\frac{\lVert \bm{x}-\bm{z}\rVert ^ \gamma}{\bm{\sigma}})$ 
% \end{center}
% where $\bm{\sigma}$ is the kernel bandwidth. When $\gamma=2$, it becomes Gaussian kernel, and when $\gamma=1$, it is Laplacian. Since different noise conditions have different stability and they may require different distance measure. Introducing an adaptive $\gamma$ enables it reach a better solution by searching a richer space.

% \subsection{Soft Thresholding by Invertible Transform}
% Note that IRM is in the range of $[0, 1]$. When using IRM as training target, the model's output should also be bounded in $[0, 1]$. With sigmoid as activation function of output layer, DNNs fulfill this constraint easily. However, because of the result from a linear sum of kernel features, the original output of kernel methods is not in $[0, 1]$. We propose to use a pair of invertible transforms to decrease the gap between training target and model's output. One pair of good candidates is logit function and sigmoid function.

% First, we use logit function 

% \begin{center}
% $\bm{y}^\prime = \frac{1}{a} (log(\frac{\bm{y}}{1-\bm{y}}) + c)$,
% \end{center}
% to transfer the original training target $y$ within (0,1) to $y\prime$ which has no range constraint, where $a$, $c$ are adjustable parameters. Then after getting kernels' output, we use sigmoid function
% \begin{center}
% $\hat{\bm{y}}^\prime = \frac{1}{1+exp(-a\hat{\bm{y}} + c)}$
% \end{center}
% to transform the estimated output $\hat{\bm{y}}$, which has no bound, into bounded $\hat{\bm{y}}^\prime$. 

% This regime serves as a soft thresholding method for the kernel output, and by choosing suitable invertible transformations, it can be used to any tasks with bounded training targets.  

==> ssn0.tex <==
\begin{figure}
\includegraphics[width=0.5\textwidth]{mulK.jpg}
\vspace{-5mm}
\caption{MSE along per frequency channel}
\label{fig:ssn0}
\vspace{-7mm}
\end{figure} 

==> subband-kernel.tex <==
\begin{table}[]
\centering
\caption{Single kernel and subband kernels}
\vspace{-3mm}
\resizebox{.8\columnwidth}{!}{
\begin{tabular}{|l|l|c|c|c|}
\hline
\multicolumn{2}{|c|}{System}                                                    & \begin{tabular}[c]{@{}c@{}}single \\kernel \end{tabular} & \begin{tabular}[c]{@{}c@{}} subband \\kernels \end{tabular} & DNN           \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}SSN\\ 0dB\end{tabular}}       & MSE  & 1.60                                                            & \textbf{1.48}                                                   & 1.67          \\ \cline{2-5} 
                                                                         & STOI & 0.81                                                            & \textbf{0.82}                                                   & \textbf{0.82} \\ \cline{2-5} 
                                                                         & PESQ & 2.35                                                            & \textbf{2.36}                                                   & 2.32          \\ \hline
                                                                         \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}SSN\\ -5dB\end{tabular}}      & MSE  & 1.67                                                            & \textbf{1.60}                                                   & 1.76          \\ \cline{2-5} 
                                                                         & STOI & 0.73                                                            & \textbf{0.74}                                                   & \textbf{0.74} \\ \cline{2-5} 
                                                                         & PESQ & 2.01                                                            & \textbf{2.03}                                                   & 2.00          \\ \hline
                                                                         \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}factory1\\ -5dB\end{tabular}} & MSE  & 2.76                                                            & \textbf{2.71}                                                   & 2.77          \\ \cline{2-5} 
                                                                         & STOI & 0.67                                                            & \textbf{0.68}                                                   & \textbf{0.68} \\ \cline{2-5} 
                                                                         & PESQ & \textbf{1.78}                                                   & 1.77                                                            & \textbf{1.78} \\ \hline
\end{tabular}
}
\vspace{-5mm}
\end{table}


==> timit_result.tex <==
\begin{table*}[htb]
\centering
\caption{Kernel \& DNN on TIMIT}
\begin{tabular}{|l|l||c|c|c||c|c|c||c|c|c|}
\hline
\multicolumn{2}{|c||}{\multirow{2}{*}{System}}     & \multicolumn{3}{c||}{5 dB}    & \multicolumn{3}{c||}{0 dB}    & \multicolumn{3}{c|}{-5 dB}   \\ \cline{3-11} 
\multicolumn{2}{|c||}{}    & Noisy & DNN  & Kernel        & Noisy & DNN  & Kernel        & Noisy & DNN  & Kernel        \\ \hline
\multirow{3}{*}{Engine}   & MSE ($\cdot 10^{-2}$) & -     & 1.41 & \textbf{1.14} & -     & 1.86 & \textbf{1.34} & -     & 1.82 & \textbf{1.17} \\ \cline{2-11} 
                          & STOI                  & 0.80  & 0.90 & \textbf{0.91} & 0.68  & 0.86 & \textbf{0.86} & 0.57  & 0.80 & \textbf{0.80} \\ \cline{2-11} 
                          & PESQ                  & 1.97  & 2.75 & \textbf{2.77} & 1.66  & 2.48 & \textbf{2.51} & 1.41  & 2.17 & \textbf{2.19} \\ \hline\hline
\multirow{3}{*}{Babble}   & MSE ($\cdot 10^{-2}$) & -     & 3.49 & \textbf{3.34} & -     & 4.37 & \textbf{4.18} & -     & 5.43 & \textbf{4.94} \\ \cline{2-11} 
                          & STOI                  & 0.77  & 0.86 & \textbf{0.86} & 0.66  & 0.76 & \textbf{0.77} & 0.55  & 0.63 & \textbf{0.64} \\ \cline{2-11} 
                          & PESQ                  & 2.08  & 2.47 & \textbf{2.52} & 1.73  & 2.05 & \textbf{2.12} & 1.42  & 1.64 & \textbf{1.70} \\ \hline\hline
\multirow{3}{*}{SSN}      & MSE ($\cdot 10^{-2}$) & -     & 1.53 & \textbf{1.35} & -     & 1.67 & \textbf{1.48} & -     & 1.76 & \textbf{1.60} \\ \cline{2-11} 
                          & STOI                  & 0.81  & 0.88 & \textbf{0.88} & 0.69  & 0.83 & \textbf{0.83} & 0.57  & 0.73 & \textbf{0.73} \\ \cline{2-11} 
                          & PESQ                  & 2.05  & 2.56 & \textbf{2.68} & 1.75  & 2.26 & \textbf{2.36} & 1.48  & 1.87 & \textbf{2.00} \\ \hline\hline
\multirow{3}{*}{Oproom}   & MSE ($\cdot 10^{-2}$) & -     & 1.85 & \textbf{1.44} & -     & 1.86 & \textbf{1.34} & -     & 1.82 & \textbf{1.17} \\ \cline{2-11} 
                          & STOI                  & 0.79  & 0.88 & \textbf{0.88} & 0.70  & 0.84 & \textbf{0.84} & 0.59  & 0.79 & \textbf{0.79} \\ \cline{2-11} 
                          & PESQ                  & 2.16  & 2.77 & \textbf{2.80} & 1.78  & 2.47 & \textbf{2.50} & 1.40  & 2.19 & \textbf{2.23} \\ \hline\hline
\multirow{3}{*}{Factory1} & MSE ($\cdot 10^{-2}$) & -     & 2.53 & \textbf{2.51} & -     & 2.55 & \textbf{2.52} & -     & 2.77 & \textbf{2.71} \\ \cline{2-11} 
                          & STOI                  & 0.77  & 0.86 & \textbf{0.86} & 0.65  & 0.78 & \textbf{0.78} & 0.54  & 0.67 & \textbf{0.68} \\ \cline{2-11} 
                          & PESQ                  & 1.99  & 2.51 & \textbf{2.56} & 1.62  & 2.17 & \textbf{2.18} & 1.29  & 1.75 & \textbf{1.82} \\ \hline
\end{tabular}
\end{table*}

==> wrap_mulK.tex <==
\begin{wrapfigure}{r}{0.25\textwidth}
  \vspace{-4mm}
  \includegraphics[width=.25\textwidth]{mulK.jpg}
    \vspace{-6mm}
\caption{MSE along per frequency channel}
  \label{fig:adaptive_vs_original}
\vspace{-5mm}
\end{wrapfigure}
